Extending Acyclicity Notions for Existential Rules (\emph{long version})

Existential rules have been proposed for representing ontological knowledge, specifically in the context of Ontology-Based Query Answering. Entailment with existential rules is undecidable. We focus in this paper on conditions that ensure the termination of a breadth-first forward chaining algorithm known as the chase. First, we propose a new tool that allows to extend existing acyclicity conditions ensuring chase termination, while keeping good complexity properties. Second, we consider the extension to existential rules with nonmonotonic negation under stable model semantics and further extend acyclicity results obtained in the positive case.

==> src/content/title.tex <==
% title.tex

\maketitle



==> src/content/tmp.tex <==
% tmp.tex


\begin{definition}[XPG]
	Let $R$ be a rule.

	Its associated position graph $\XPG{R}$ is a graph where
	\begin{itemize}
	\item there is a vertex $\vxpg{x}{p}{i}{a}$ for each position $i$
	in an atom $a$, where $x$ is the term occuring in this position and
	$p$ the atom predicate ;
	\item for each $\vxpg{x}{p}{i}{a}$ in the frontier,
	there is a {\em normal} edge to each $\vxpg{x}{p'}{i'}{a'}$ in the head,
	and a {\em special} edge to each $\vxpg{z}{p'}{i'}{a'}$ where $z$ is an existentially
	quantified variable.
	\end{itemize}

	If $\R$ is a set of rules, the $\XPG{\R}$ is defined as the disjoint union
	of all $\XPG{R_i}, \forall R_i \in \R$.
\end{definition}

%Sans doute mieux si d'abord 'PG' pour une seule règle, puis on passe au XPG,
%comme l'union, puis ensuite on parle des FPG, DPG et UPG.
%\begin{definition}[XPG]
%	Let $\R$ be a set of rules.
%
%	Its associated $\XPG{\R}$ is a graph with one vertex
%	$\vxpg{x}{p}{i}{a}$ for each rule $R_i \in \R$, for each
%	position $i$ in an atom $a$, where $p$ indicates the
%	predicate of $a$ and $x$ the term occuring in this position.
%
%	For each $\vxpg{x}{p}{i}{a}$ in the body of a rule $R_i$,
%	there is a {\em normal} edge to each $\vxpg{x}{p'}{i'}{a'}$ in the head of $R_i$,
%	and a {\em special} edge to each $\vxpg{z}{p'}{i'}{a'}$ in $R_i$ where $z$ is an existentially
%	quantified variable.
%
%	The $X$ in $XPG$ determines the edges between different rules.
%\end{definition}

\begin{definition}[FPG]
	Let $\R$ be a set of rules.

	The $\FPG{\R}$ is the $\XPG{\R}$ where
	one edge is added for each $\vxpg{x}{p}{i}{a}$ in a rule head 
	to each $\vxpg{x'}{p}{i}{a'}$ in a rule body.
\end{definition}

\begin{definition}[DPG]
	Let $\R$ be a set of rules.

	The $\DPG{\R}$ is the $\XPG{\R}$ where
	one edge is added for each $\vxpg{x}{p}{i}{a}$ in a rule head $H_i$
	to each $\vxpg{x'}{p}{i}{a'}$ in a rule body $B_j$ if there is a
	unifier of $B_j$ with $H_i$.
\end{definition}

\begin{definition}[UPG]
	Let $\R$ be a set of rules.

	The $\UPG{\R}$ is the $\XPG{\R}$ where
	one edge is added for each $\vxpg{x}{p}{i}{a}$ in a rule head $H_i$
	to each $\vxpg{x'}{p}{i}{a'}$ in a rule body $B_j$ if there is a
	unifier $\unifier$ of $B_j$ with $H_i$ such that $\unifier(x) = \unifier(x')$.
\end{definition}

\begin{proposition}
	$\R$ satisfies $\grd{Y}$ iff $\DPG{\R}$ satisfies $Y$.
\end{proposition}

\begin{definition}[Cycle property]


Penser à :\\
If $\XPG{\R}$ satisfies $Y$, then for all $X'PG(\R)$ with $E_\unifier(X') \subseteq E_\unifier(X)$,
$X'PG(\R)$ satisfies $Y$.
\end{definition}

\begin{proposition}
\label{prop:y-strict-ygrd}
	Let $Y$ be a cycle property.
	If $\agrd \nsubseteq Y$ then $Y \subset \grd{Y}$.
\end{proposition}

\begin{preuve}
	Let $Y$ be a cycle property such that $\agrd \nsubseteq Y$.
	Then, there is a set of rules $\R$ which satisfies $\agrd$
	but does not satisfy $Y$.
	Since $\grd{Y}$ generalises $\agrd$, $\R$ belongs to
	$\grd{Y}$.
\end{preuve}

\begin{proposition}
\label{prop:ygrd-strict-ygerd}
	Let $Y$ be a cycle property.
	If $Y \subset \grd{Y}$ then $\grd{Y} \subset \gerd{Y}$.
\end{proposition}

\begin{preuve}
	Let $Y$ be a cycle property such that $Y \subset \grd{Y}$
	and $\R$ be a set of rules which satisfies $\grd{Y}$ but does not
	satisfy $Y$.

	$\R$ can be rewrite in $\R'$ by applying the following steps.

	First, for each rule $R_i = B_i[\X,\Y] \rightarrow H_i[\Y,\Z] \in \R$,
	let $R_{i,1} = B_i[\X,\Y] \rightarrow p_i(\X,\Y)$ where $p_i$ is a fresh
	predicate ; and $R_{i,2} = p_i(\X,\Y) \rightarrow H_i[\Y,\Z]$.
	%Then for each pair of rules $R_{i,2},R_{j,1}$

	Then, for each rule $R_{i,1}$, let $R'_{i,1}$ be the rule $(B'_{i,1},H_{i,1})$
	with $B'_{i,1} = B_{i,1} \cup \{p'_{j,i}(x_{j,i}) : \forall R_{j} \in \R\}$,
	where $p'_{j,i}$ are fresh predicates and $x_{j,i}$ fresh variables.

	Now, for each rule $R_{i,2}$ let $R'_{i,2}$ be the rule $(B_{i,2},H'_{i,2})$
	with $H'_{i,2} = H_{i,2} \cup \{p'_{i,j}(z_{i,j}) : \forall R_{j} \in \R\}$,
	where $z_{i,j}$ are fresh existentially quantified variables.

	Let $\R' = \bigcup\limits_{R_i \in \R} R'_{i,1},R'_{i,2}$.

	Since this construction ensures that there is at least one unifier of each
	rule $R'_{i,1}$ with each rule $R'_{j,2}$ and of each rule $R'_{i,2}$ with $R'_{i,1}$,
	the $\DPG{\R'}$ contains exactly one cycle for each cycle in the $\FPG{\R}$.

	So, $\DPG{\R'}$ contains at least one cycle which does not satisfy $Y$,
	and then $\R'$ is not $\grd{Y}$.

	But one can also see that $\UPG{\R'}$ contains the same cycles than
	$\DPG{\R}$, and since $\DPG{\R}$ verifies $Y$, $\UPG{\R'}$ also does.

	Hence, $\R'$ is a set of rules which does not belong to $\grd{Y}$
	but to $\gerd{Y}$.
\end{preuve}

\begin{observation}
	The {\em jump} between $Y$ and $\grd{Y}$ is at least the {\em same} than
	between $\grd{Y}$ and $\gerd{Y}$.
\end{observation}

\begin{proposition}
	Let $Y_1,Y_2$ be two cycle properties.
	If $Y_1 \subseteq Y_2$,
	then $\grd{Y_1} \subseteq \grd{Y_2}$.
\end{proposition}

\begin{preuve}[necessaire ?]
	%Obviously, $Y_1 \subseteq \grd{Y_1}$ and $Y_2 \subseteq \grd{Y_2}$.
	Each S.C.C. of any set of rules $\R \in \grd{Y_1}$ satisfies
	$Y_1$, it also satisfies $Y_2$.
	Hence $\R$ is $\grd{Y_2}$.
\end{preuve}

%\begin{proposition}
%	Let $Y_1, Y_2$ be two cycle properties such that:
%	\begin{itemize}
%		%\item $\agrd \nsubseteq Y_2$,	%replace by def
%		\item $Y_2 \neq \grd{Y_1}$		% otherwise, we cannot get a complete GRD which matches def
%		\item $Y_2 \nsubseteq \agrd$,	% to ensure that transformation conserves Y_2
%		\item $Y_1 \subset Y_2$,
%		\item $\wa \subseteq Y_1$.		% need for transformation
%	\end{itemize}
%	Then $\grd{Y_1} \subset \grd{Y_2}$.
%\end{proposition}
%
%\begin{preuve}
%	Let $\R$ be a set of rules such that $\R$ satisfies $Y_2$ and %does not
%	%satisfy $Y_1$.
%	neither $Y_1$ nor $\agrd$.
%
%	$\R$ can be rewrited in $\R'$, by replacing each rule $R_i = (B_i,H_i) \in \R$
%	with a new rule $R'_i = (B_i \cup \{p(x)\}, H_i \cup \{p(x)\})$ where
%	$p$ is a fresh predicate, and $x$ a fresh variable.
%
%	Each rule may now be unified with any other rule,
%	but the only circuits which are created are those which contains only atoms
%	$p(x)$, hence no special edge is contained in any of those circuits.
%
%	Since $\wa \subseteq Y_1$ (and so $\wa \subseteq Y_2$), the added circuit does
%	not change satisfiability of $Y_1$ and $Y_2$.
%	Before rewriting there was at least one circuit which did not satisfy $Y_1$, while
%	all circuits satisfied $Y_2$.
%
%	And one can see that $\DPG{\R'}$ contains the same cycles as $\FPG{\R}$.
%	Hence, $\R'$ is $\grd{Y_2}$ but is not $\grd{Y_1}$.
%\end{preuve}

\begin{proposition}[version 2]
	Let $Y_1, Y_2$ be two cycle properties such that:
	\begin{itemize}
		%\item $\agrd \nsubseteq Y_2$,	% ? not needed since we take a complete GRD
		\item $Y_2 \neq \grd{Y_1}$		% otherwise, we cannot get a complete GRD which matches def
		\item $Y_2 \nsubseteq \agrd$,	% otherwise pb to find a correct seet of rules
		\item $Y_1 \subset Y_2$,		% obvious
		%\item $\wa \subseteq Y_1$.
	\end{itemize}
	Then $\grd{Y_1} \subset \grd{Y_2}$.
\end{proposition}

\begin{preuve}
	Let $\R$ be a set of rules whose graph of rules dependencies is complete,
	which satisfy $Y_2$ and does not satisfy $Y_1$.

	Note that if we add the constraint that $\wa \subseteq Y_1$,
	such a set can be easily built from any set of rules which satisfy $Y_2$ while
	not satisfying $Y_1$ (see observation below).%\ref{obs:y1-strict-y2}).

	Obviously, this set of rules satisfy $\grd{Y_2}$.
	Since $\DPG{\R} = \FPG{\R}$, $\R$ does not satisfy $\grd{Y_1}$.
\end{preuve}

\begin{observation}
\label{obs:y1-strict-y2}
	Let $\R$ be a set of rules such that $\R$ satisfies $Y_2$ and %does not
	%satisfy $Y_1$.
	neither $Y_1$ nor $\agrd$.
	$\R$ can be rewrited in $\R'$, by replacing each rule $R_i = (B_i,H_i) \in \R$
	with a new rule $R'_i = (B_i \cup \{p(x)\}, H_i \cup \{p(x)\})$ where
	$p$ is a fresh predicate, and $x$ a fresh variable.

	Each rule may now be unified with any other rule,
	but the only circuits which are created are those which contains only atoms
	$p(x)$, hence no special edge is contained in any of those circuits.

	Since $\wa \subseteq Y_1$ (and so $\wa \subseteq Y_2$), the added circuit does
	not change satisfiability of $Y_1$ and $Y_2$.

	Hence $\R'$ is equivalent to $\R$ from the cycle properties points of view,
	and the graph of rules dependencies of $\R'$ is complete.
\end{observation}




